Classical, Machine Learning, and Hybrid Solvers for Partial Differential Equations: An Evidence-Weighted Review and Decision Framework

Machine learning for partial differential equations raises a practical question: when are classical, learned, or hybrid solvers justified? This survey compares the three families in a decision framework organized by data availability, query volume, and certification needs. An amortization law, tested on parametric Darcy flow, shows that surrogates trained on solver-generated data break even only after many queries, beyond thirty thousand for errors below one percent. An evidence ladder, a benchmark reanalysis, and three case studies show that claims of speedup and generalization carry the weakest evidence. Solver choice should follow regime, query volume, and evidence quality, not method novelty.

==> main_labels.tex <==
% Generated by tools/update_main_labels.py from main.aux. Do not edit by hand.
\mainlabel{eq:amortization_law}{1}
\mainlabel{sec:benchmark_landscape}{4}
\mainlabel{sec:case_studies}{5}
\mainlabel{sec:decision_matrix}{6}
\mainlabel{sec:open_problems}{7}
\mainlabel{sec:taxonomy}{2}
\mainlabel{subsec:benchmark_suites}{4.1}
\mainlabel{subsec:case_audits}{5.2}
\mainlabel{subsec:case_gon}{5.1}
\mainlabel{subsec:cost_comparison}{4.4}
\mainlabel{subsec:evidence_rubric}{4.7}
\mainlabel{subsec:function_learning}{3.2.1}
\mainlabel{subsec:measured_nstar}{4.6}
\mainlabel{subsec:operator_learning}{3.2.2}
\mainlabel{tab:decision_matrix}{13}
\mainlabel{tab:evidence_rubric}{9}
\mainlabel{tab:measured_nstar}{8}

